RHH-LGP: Receding Horizon And Heuristics-Based Logic-Geometric Programming For Task And Motion Planning

Sequential decision-making and motion planning for robotic manipulation induce combinatorial complexity. For long-horizon tasks, especially when the environment comprises many objects that can be interacted with, planning efficiency becomes even more important. To plan such long-horizon tasks, we present the RHH-LGP algorithm for combined task and motion planning (TAMP). First, we propose a TAMP approach (based on Logic-Geometric Programming) that effectively uses geometry-based heuristics for solving long-horizon manipulation tasks. The efficiency of this planner is then further improved by a receding horizon formulation, resulting in RHH-LGP. We demonstrate the robustness and effectiveness of our approach on a diverse range of long-horizon tasks that require reasoning about interactions with a large number of objects. Using our framework, we can solve tasks that require multiple robots, including a mobile robot and snake-like walking robots, to form novel heterogeneous kinematic structures autonomously. By combining geometry-based heuristics with iterative planning, our approach brings an order-of-magnitude reduction of planning time in all investigated problems.

==> img/modules.tex <==
\begin{figure*}[t]
    \centering
    \caption{The robot modules used in the present work and their configurations.}\label{fig:modules}
\end{figure*}

==> old/relatedWork.tex <==
%\oz{let's keep RW at max 1 column length, or maybe even bury it in the intro if possible.}
% \subsection{Modular robotics}
% \cor{this can go tot the intro as it simply motivates the present work}
% % autonomy
% So far, only few works addressed the challenges related to fully autonomous TAMP for modular robots.
% Daudelin et al. \cite{daudelin2018integrated}, presented a modular robot system, which is able indeed able to plan and perform actions autonomously.
% However, the system still uses closed loop control for behaviors, which restricts its capacities to very simple tasks.
% In particular, the high-level task planner of this work is still not integrating a motion planner into the planning process, so this system does not perform integrated TAMP.
% In fact, to this day, we are not aware of any modular robot system that uses combined TAMP to plan and execute a long sequence of actions autonomously in order to reach one or multiple long-term goals.
% %
% reconfigurability related to TAMP
% Another facet of modular robot autonomy is self-reconfigurability.
% Autonomous reconfiguration remains one of the biggest challenges for modular robots and most of the previous works solely focuses one of those aspects. 
% So far, we are only aware of one system, which performs all three steps of the self-reconfiguration pipeline autonomously \cite{daudelin2018integrated}.
% As stated above though, this systems capacities are limited and it does not perform combined TAMP in the sense that we aim to do.

% \subsection{Heuristics usage in planning}
% % Cornelius: this will be moved to the background section
% % %
% % % MBTS and that symbolic search is slow despite the bounds
% % In order to limit the computational costs of calling the motion planner, Toussaint and Lopes \cite{toussaint2017multi} combined LGP with multi-bounded tree search.
% % This method is based on the observation that the feasibility of a relaxed geometric problem is a necessary condition for the feasibility of the original motion planning problem, whilst being computationally simpler.
% % In this framework, the outputs of the relaxed motion planning problems serve as a heuristic to guide the task planning.
% % While the approach has produced some very promising results in \cite{hartmann2020robust, driess2019hierarchical}, the computation of the planning heuristic requires calling the motion planner to compute a lower bound to guide search.
% % For big problem instances this can still be problematic, as even the optimisation of relaxed geometric problems can take long time \cite{hartmann2020robust}.

% % geometry-based: Akbari; Vega-Brown; toussaint!! --> downsides!!!
% Some notable works on TAMP use \textit{geometry-based} heuristics, which leverage geometric information from the environment to improve planning performance, without calling the actual motion planner to compute a geometry-based heuristic score.
% Vega-Brown and Roy \cite{vega2018admissible} for instance, made use of geometric abstractions to effectively plan tasks. 
% In order to estimate the heuristic costs of executing an action, the authors defined upper and lower bounds of the costs for each predefined action. 
% In \cite{akbari2019combined}, the authors combined the FF planner with relaxed geometric reasoning to prune geometrically infeasible actions. 
% Their geometric reasoning procedure evaluated several geometric conditions, such as reachability and stability, on a relaxed geometrical problem without calling a motion planner, while the actual motion planner was only called when the relaxed problem was feasible.
% However, most of the previous works that used heuristics for TAMP mostly focused on smaller problem instances, which either required few actions to be solved \cite{akbari2019combined, driess2020deep} or contained few objects in the environment \cite{toussaint2017multi}.

% \subsection{Long-horizon TAMP}
% Developing a TAMP solver which can plan long-horizon tasks remains a challenging problem \cite{nair2019hierarchical,driess2021learning}.
% One technique to adapt TAMP algorithms to long-term tasks is to reduce search space size.
% We already described heuristic methods to achieve such a search space size reduction above.

% Another technique to handle the challenges of long-horizon TAMP is iterative planning, i.e.\ problem decomposition.
% Such planners only execute and plan a portion of the task at each time step.
% The benefit of this approach is that very big problems are reduced to small-scale problems which are computationally tractable.
% Some previous works have tackled long-horizon TAMP by defining several sub-goals that have to be fulfilled in order to complete an entire long-horizon task \cite{nair2019hierarchical, gupta2019relay}.
% For instance, Castamann et al. \cite{castaman2020receding} adapted the model predictive control, i.e.\ RHC algorithm, to TAMP.
% In each planning iteration a fixed number of actions was planned, but only the first action of each plan was in fact executed.
% In difference to that, Hartman et al. \cite{hartmann2020robust} predefined a number of actions that was planned and executed in each iteration of the planning algorithm.
% The latter work is most similar to the receding horizon LGP solver that we present in the present paper.


==> tables/constraints.tex <==
\begin{table}[ht]
\resizebox{\linewidth}{!}{\begin{tabularx}{\linewidth}{l|l}
    \multicolumn{1}{c|}{\textbf{Predicate}}      & \multicolumn{1}{c}{\textbf{Constraints}} \\[0.5em] \hline \\\relax
    [touch X Y]             & the distance between X and Y equals 0       \\[0.7em]
    [stable X Y]            & create a stable joint from X to Y,\\
                            & constrained to velocity 0 \\[0.7em]
    [above X Y]             & X is above Y with a distance of $> 0$ \\[0.7em]
    [connectCrawlers X Y]   & the distance between the effectors X and Y is 0 \\
                            & the z-vectors of the effectors oppose each other,\\
                            & the other two axes are perpendicular     \\[0.7em]
    [touchBoxNormal X Y]    & the distance between X and Y equals 0\\
                            & the z-axis of object X points upwards\\
                            & the z-axis of X and the x-axis of Y are perpendicular\\[0.5em]
\end{tabularx}}
\caption{Predicates to constrain trajectory optimisation.}\label{tbl:constraints}
\end{table}

==> tables/exp2.tex <==
\begin{table}[htbp]
\centering
\begin{tabular} {@{}rrrrr@{}} \toprule
$n$ & Time in s. & \# Tree nodes & \# Expanded & Sol. len. \\
\midrule
1       & 11.81     & 576       & 77        & 11 \\
2       & 111.39    & 1197      & 153       & 14 \\
4       & 151.42    & 1375      & 145       & 12 \\
8       & 30.90     & 1157      & 77        & 12 \\
\bottomrule
\end{tabular}
\caption{Climbing task with multiple goals planned with MBTS + action-specific heuristics.}\label{tbl:complex}
\end{table}

==> tables/exp3.tex <==
\begin{table*}[htbp]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular} {@{}rrrrrcrrrr@{}} \toprule
\multicolumn{1}{c}{$n$} & \multicolumn{4}{c}{One crawler} & \phantom{abc} & \multicolumn{4}{c}{Two crawlers} \\
\cmidrule{2-5} \cmidrule{7-10} & Time in s. & \# Tree nodes & \# Expanded & Sol. len. && Time in s. & \# Tree nodes & \# Expanded & Sol. len. \\
\midrule
1       & 0.08      & 10        & 2         & 2  && 0.48        & 21      & 3         & 2 \\
2       & 0.56      & 49        & 11        & 5  && 7.00        & 81      & 13        & 2 \\
4       & 2.69      & 85        & 13        & 7  && 13.59       & 190     & 22        & 8 \\
8       & 3.61      & 181       & 17        & 10 && 11.64       & 309     & 23        & 9 \\
16      & 22.41     & 505       & 27        & 16 && 16.38       & 590     & 26        & 11 \\
32      & 444.26    & 5849      & 171       & 50 && 138.03      & 2066    & 47        & 19 \\
64      & --        & --        & --        & -- && 439.01      & 4088    & 53        & 27 \\
\bottomrule
\multicolumn{10}{l}{\footnotesize Note: scenarios without metrics could not be solved at all}\\
\end{tabular}}
\caption{Planning the climbing task using MBTS and action-specific heuristics for different numbers of available modules.}\label{tbl:exp3}
\end{table*}

==> tables/exp4.tex <==
\begin{table}[htbp]
\centering
\begin{tabular} {@{}rrrrr@{}} \toprule
$n$ & Time in s. & Tree nodes & Expanded nodes & Solution len. \\
\midrule
1       & 1.84      & 7        & 2      & 3  \\
2       & 2.18      & 12       & 4      & 5  \\
4       & 3.45      & 25       & 8      & 9 \\
8       & 17.40     & 63       & 16     & 17 \\
\bottomrule
\end{tabular}
\caption{Modular robot pick-and-place task planned with MBTS and action-specific heuristics.}\label{tbl:exp4}
\end{table}


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

